xMem: A CPU-Based Approach for Accurate Estimation of GPU Memory in Deep Learning Training Workloads

The global scarcity of GPUs necessitates more sophisticated strategies for Deep Learning jobs in shared cluster environments. Accurate estimation of how much GPU memory a job will require is fundamental to enabling advanced scheduling and GPU sharing, which helps prevent out-of-memory (OOM) errors and resource underutilization. However, existing estimation methods have limitations. Approaches relying on static analysis or historical data with machine learning often fail to accurately capture runtime dynamics. Furthermore, direct GPU analysis consumes scarce resources, and some techniques require intrusive code modifications. Thus, the key challenge lies in precisely estimating dynamic memory requirements, including memory allocator nuances, without consuming GPU resources and non-intrusive code changes. To address this challenge, we propose xMem, a novel framework that leverages CPU-only dynamic analysis to accurately estimate peak GPU memory requirements a priori. We conducted a thorough evaluation of xMem against state-of-the-art solutions using workloads from 25 different models, including architectures like Convolutional Neural Networks and Transformers. The analysis of 5209 runs, which includes ANOVA and Monte Carlo results, highlights xMem's benefits: it decreases the median relative error by 91% and significantly reduces the probability of estimation failure as safe OOM thresholds by 75%, meaning that the estimated value can often be used directly without causing OOM. Ultimately, these improvements lead to a 368% increase in memory conservation potential over current solutions.

==> preamble.tex <==
% \newcommand{\subparagraph}{} % hack for ieeetran bug with titlesec package
% \usepackage[moderate,tracking=normal]{savetrees} % subtle moderate extreme
% \renewcommand*\ttdefault{txtt}
\renewcommand*\ttdefault{lmvtt}
% \usepackage[inkscapelatex=false]{svg}
% \usepackage{todonotes}
% \usepackage{listings}
% \hypersetup{colorlinks,linkcolor=blue}
\usepackage{url}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{subfiles}
% \usepackage{cite}
% \usepackage{amsmath,amssymb,amsfonts}
% \usepackage{ifthen}
% \usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{textcomp}
\usepackage[table]{xcolor}
\definecolor{stripe}{RGB}{254,254,217}
% for circled numbers
\usepackage{pifont}
\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle, draw, inner sep=1pt] (char) {#1};}}
% {230, 253, 248}
% {212,251,243}
\definecolor{exp-xMem}{HTML}{377eb8}
\definecolor{exp-DNNMem}{HTML}{e41a1c}
\definecolor{exp-SchedTune}{HTML}{4daf4a}
\definecolor{exp-LLMem}{HTML}{984ea3}
\definecolor{fq-bl}{HTML}{2C7BB6}
\definecolor{fq-br}{HTML}{FDAE61}
\definecolor{fq-tl}{HTML}{ABD9E9}
\definecolor{fq-tr}{HTML}{D7191C}



\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\usepackage{colortbl}
\usepackage{array}
\usepackage{booktabs}
\newcommand{\midsepremove}{\aboverulesep=0mm \belowrulesep=0mm}
\midsepremove
\newcommand{\midsepdefault}{\aboverulesep=0mm \belowrulesep=0mm}
\midsepdefault

\usepackage[inline]{enumitem}
	\setlist[enumerate]{leftmargin=1.2em}%itemsep=0.33em
	\setlist[itemize]{leftmargin=1.2em,label={$\bullet$}}%



% Command list
% \renewcommand{\lstlistingname}{Code} % Change "Listing" to "Code"

\newcommand{\projectname}{xMem\@\xspace}
\newcommand{\imagePath}{assets}
\newcommand{\xmemtotalevaruns}{5209\@\xspace}
\newcommand{\xmemprobability}{13\%\@\xspace}
\newcommand{\xmemmemory}{4 GB\@\xspace}
\newcommand{\xmemmedianerror}{5\%\@\xspace}
\newcommand{\xmemruntime}{12s\@\xspace}

\newcommand{\xmemmedianerrorimprove}{91\%\@\xspace}
\newcommand{\xmemprobabilityimprove}{75\%\@\xspace}
\newcommand{\xmemmemoryimprove}{368\%\@\xspace}
\newcommand{\xmemruntimeimprove}{-110\%\@\xspace}




%%% abbreviation macros - begin
\usepackage{xspace}
\newcommand*{\aka}{{aka}\@\xspace}
\newcommand*{\cf}{\textit{cf.}\@\xspace}
\newcommand*{\eg}{\textit{e.g.,}\@\xspace}
\newcommand*{\ie}{\textit{i.e.,}\@\xspace}
\makeatletter
\newcommand*{\etc}{%
    \@ifnextchar{.}%
        {etc}%
        {etc.\@\xspace}%
}
\newcommand*{\etal}{%
    \@ifnextchar{.}%
        {et al}%
        {et al.\@\xspace}%
}
\makeatother


